Multi-output Headed Ensembles for Product Item Classification

In this paper, we revisit the problem of product item classification for large-scale e-commerce catalogs. The taxonomy of e-commerce catalogs consists of thousands of genres to which are assigned items that are uploaded by merchants on a continuous basis. The genre assignments by merchants are often wrong but treated as ground truth labels in automatically generated training sets, thus creating a feedback loop that leads to poorer model quality over time. This problem of taxonomy classification becomes highly pronounced due to the unavailability of sizable curated training sets. Under such a scenario it is common to combine multiple classifiers to combat poor generalization performance from a single classifier. We propose an extensible deep learning based classification model framework that benefits from the simplicity and robustness of averaging ensembles and fusion based classifiers. We are also able to use metadata features and low-level feature engineering to boost classification performance. We show these improvements against robust industry standard baseline models that employ hyperparameter optimization. Additionally, due to continuous insertion, deletion and updates to real-world high-volume e-commerce catalogs, assessing model performance for deployment using A/B testing and/or manual annotation becomes a bottleneck. To this end, we also propose a novel way to evaluate model performance using user sessions that provides better insights in addition to traditional measures of precision and recall.

==> src/related-work.tex <==
\section{Related Work}
\label{section:related-work}

\begin{tcolorbox}
[
  enhanced,
  attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=red!5!white,
  colframe=red!75!black,
  colbacktitle=red!80!black,
  fonttitle=\bfseries,
  boxed title style={size=small,colframe=red!75!black},
  title=Speed! Speed! Speed!
]
@Arthur, please fill in your bibliography on user behavior driven evaluations here.
Some references can come from \url{https://www.hongliangjie.com/data-science-at-etsy/} for ideas and references.
\end{tcolorbox}


==> src/tables/tab-baseline_performance_2level.tex <==
	    \begin{tabular*}{\textwidth}{|c|c|c||c|c|}
	    \cline{1-5}
	    & Data Size & N Class & FastText & MoHE \\
	    \hhline{|=|==||==|}
	    Home Decor & \makecell[r]{1260798} & \makecell[r]{310} & 0.763 & 0.774 \\
	    \cline{1-5}
	    Foods & \makecell[r]{461963} & \makecell[r]{880} & 0.686 & 0.730 \\
	    \cline{1-5}
	    Healthcare \& Med. Supplies & \makecell[r]{420776} & \makecell[r]{381} & 0.677 & 0.752 \\
	    \cline{1-5}
	    Shoes & \makecell[r]{340078} & \makecell[r]{80} & 0.710 & 0.708 \\
	    \cline{1-5}
	    Computers \& Networking & \makecell[r]{384861} & \makecell[r]{263} & 0.628 & 0.675 \\
	    \cline{1-5}
	    Beverages & \makecell[r]{178114} & \makecell[r]{42} & 0.799 & 0.807 \\
	    \cline{1-5}
	    Professional Services & \makecell[r]{49964} & \makecell[r]{85} & 0.462 & 0.719 \\
	    \cline{1-5}
	    Cars \& Motorcycles & \makecell[r]{7088} & \makecell[r]{217} & 0.025 & 0.883 \\
	    \cline{1-5}
	    Fiber-Optic/Mobile Comm. & \makecell[r]{1937} & \makecell[r]{10} & 0.375 & 0.642 \\
	    \hhline{|=|==||==|}
	    All Genres & 23701953 & 11397 & 0.637 & 0.700 \\
	    \cline{1-5}
	    \end{tabular*}

==> src/tables/tab-meta_performance_2level.tex <==
	    \begin{tabular*}{\textwidth}{|c|c|c|c|c|c|c|c|}
	    \cline{1-8}
	     & Baseline & Shop ID & Tag ID & Shop/Tag ID & desc-append & desc-aux & Shop/Tag ID + desc-aux\\
	    \hhline{|========|}
        \cline{1-8}
	    Home Decor & 0.774 & 0.784 & 0.793 & 0.801 & 0.780 & 0.779 & 0.800 \\
	    \cline{1-8}
	    Foods & 0.730 & 0.746 & 0.754 & 0.759 & 0.744 & 0.745 & 0.766 \\
	    \cline{1-8}
	    Healthcare \& Med. Supplies & 0.752 & 0.776 & 0.767 & 0.790 & 0.781 & 0.783 & 0.798 \\
	    \cline{1-8}
	    Shoes & 0.708 & 0.719 & 0.722 & 0.733 & 0.726 & 0.725 & 0.736 \\
	    \cline{1-8}
	    Computers \& Networking & 0.675 & 0.689 & 0.673 & 0.689 & 0.679 & 0.673 & 0.689 \\
	    \cline{1-8}
	    Beverages & 0.807 & 0.811 & 0.816 & 0.822 & 0.817 & 0.817 & 0.833 \\
	    \cline{1-8}
	    Professional Services & 0.719 & 0.728 & 0.716 & 0.723 & 0.725 & 0.722 & 0.739 \\
	    \cline{1-8}
	    Cars \& Motorcycles & 0.883 & 0.866 & 0.889 & 0.865 & 0.866 & 0.870 & 0.866 \\
	    \cline{1-8}
	    Fiber-Optic/Mobile Comm. & 0.642 & 0.692 & 0.670 & 0.621 & 0.673 & 0.620 & 0.706 \\
        \hhline{|========|}
	    All & 0.700 & 0.712 & 0.708 & 0.719 & 0.715 & 0.712 & 0.723 \\
	    \cline{1-8}
	    \end{tabular*}



==> src/tables/tab-mof-keywords.tex <==
\begin{tabular*}{\textwidth}{|c|c|c|}
\cline{1-3}
Genre Name & Shop/TagID & Shop/TagID/Keywords\\
\hhline{|===|}
*Fiber-Optic Comm. \& Mobile Comm. & 0.770 & 0.909 (↑↑)\\
\cline{1-3}
*Cars \& Motorcycles & 0.905 & 0.934 (↑↑)\\
\cline{1-3}
Catalog Gifts \& Tickets & 0.844 & 0.839 (↓)\\
\cline{1-3}
*Professional Services & 0.833 & 0.849 (↑↑)\\
\cline{1-3}
Video Games & 0.853 & 0.876 (↑↑)\\
\cline{1-3}
Japanese Sake \& Shochu & 0.876 & 0.875 (↓)\\
\cline{1-3}
Watches & 0.863 & 0.865 (↑)\\
\cline{1-3}
Musical Instruments & 0.767 & 0.769 (↑)\\
\cline{1-3}
Sweets \& Snacks & 0.788 & 0.789 (↑)\\
\cline{1-3}
*Beverages & 0.852 & 0.846 (↓)\\
\cline{1-3}
Alcoholic Beverages & 0.758 & 0.769 (↑↑)\\
\cline{1-3}
Underwear, Socks \& Sleepwear & 0.786 & 0.788 (↑)\\
\cline{1-3}
TVs, Audio \& Cameras & 0.733 & 0.736 (↑)\\
\cline{1-3}
Toys \& Games & 0.772 & 0.777 (↑)\\
\cline{1-3}
Diet \& Health & 0.743 & 0.743 (→)\\
\cline{1-3}
Appliances & 0.799 & 0.798 (↓)\\
\cline{1-3}
*Shoes & 0.749 & 0.750 (↑)\\
\cline{1-3}
*Computers \& Networking & 0.724 & 0.730 (↑)\\
\cline{1-3}
*Healthcare \& Medical Supplies & 0.822 & 0.828 (↑)\\
\cline{1-3}
*Foods & 0.774 & 0.776 (↑)\\
\cline{1-3}
Jewelry \& Accessories & 0.805 & 0.809 (↑)\\
\cline{1-3}
Pets \& Pet Supplies & 0.791 & 0.797 (↑)\\
\cline{1-3}
Men's Fashion & 0.878 & 0.877 (↓)\\
\cline{1-3}
Kids, Baby \& Maternity & 0.801 & 0.802 (↑) \\
\cline{1-3}
Women's Fashion & 0.859 & 0.861 (↑) \\
\cline{1-3}
Smartphones \& Tablet PCs & 0.841 & 0.851 (↑↑) \\
\cline{1-3}
Bags \& Fashion Accessories & 0.813 & 0.809 (↓) \\
\cline{1-3}
Beauty, Cosmetics \& Fragrances & 0.763 & 0.763 (→) \\
\cline{1-3}
Music \& Video & 0.604 & 0.605 (↑) \\
\cline{1-3}
Hobbies & 0.836 & 0.832 (↓) \\
\cline{1-3}
Kitchen, Dining \& Bar & 0.811 & 0.811 (→) \\
\cline{1-3}
*Home Decor, Bedding \& Storage Furn. & 0.823 & 0.820 (↓)\\
\cline{1-3}
Sports \& Outdoors & 0.803 & 0.804 (↑) \\
\cline{1-3}
Car \& Motorcycle Supplies & 0.808 & 0.803 (↓) \\
\cline{1-3}
Flowers, Gardening \& DIY & 0.673 & 0.676 (↑) \\
\cline{1-3}
Household Goods, Stationery \& Craft & 0.823 & 0.826 (↑)\\
\cline{1-3}
Books & 0.671 & 0.672 (↑) \\
\cline{1-3}
\end{tabular*}



==> src/tables/table-identical-performance.tex <==
%	    \begin{tabular*}{\textwidth}{|c|c|c||c|c|c|c|}
%	    \cline{1-7}
%	    Categories & Data Size & N Class & MoF & Ensemble & TextCNN & MoE\\
%	    \hhline{|=|==||====|}
%	    Home Decor & \makecell[r]{1260798} & \makecell[r]{310} & \textbf{0.869} / \textbf{0.778} & 0.865 / 0.770 & 0.855 / 0.756 & 0.851 / 0.747\\
%	    \cline{1-7}
%	    Foods & \makecell[r]{461963} & \makecell[r]{880} & \textbf{0.778} / \textbf{0.740} & 0.775 / 0.733 & 0.760 / 0.717 & 0.747 / 0.700\\
%	    \cline{1-7}
%	    Healthcare \& Med. Supplies & \makecell[r]{420776} & \makecell[r]{381} & \textbf{0.841} / \textbf{0.772} & 0.834 / 0.750 & 0.822 / 0.742 & 0.819 / 0.731\\
%	    \cline{1-7}
%	    Shoes & \makecell[r]{340078} & \makecell[r]{80} & \textbf{0.810} / \textbf{0.709} & 0.801 / 0.699 & 0.782 / 0.681 & 0.784 / 0.679\\
%	    \cline{1-7}
%	    Computers \& Networking & \makecell[r]{384861} & \makecell[r]{263} & \textbf{0.858} / \textbf{0.682} & 0.850 / \textbf{0.682} & 0.842 / 0.664 & 0.841 / 0.650\\
%	    \cline{1-7}
%	    Beverages & \makecell[r]{178114} & \makecell[r]{42} & \textbf{0.893} / \textbf{0.798} & 0.886 / 0.770 & 0.876 / 0.781 & 0.876 / 0.747\\
%	    \cline{1-7}
%	    Professional Services & \makecell[r]{49964} & \makecell[r]{85} & \textbf{0.938} / 0.790 & 0.935 / \textbf{0.794} & 0.922 / 0.780 & 0.924 / 0.771\\
%	    \cline{1-7}
%	    Cars \& Motorcycles & \makecell[r]{7088} & \makecell[r]{217} & \textbf{0.968} / \textbf{0.920} & 0.965 / 0.919 & 0.965 / 0.924 & 0.958 / 0.914\\
%	    \cline{1-7}
%	    Fiber-Optic/Mobile Comm. & \makecell[r]{1937} & \makecell[r]{10} & \textbf{0.943} / \textbf{0.768} & 0.928 / 0.484 & 0.934 / 0.662 & 0.929 / 0.470\\
%	    \cline{1-7}
%	    SIGIR (English) & \makecell[r]{712761} & \makecell[r]{3008} & \textbf{0.803} / \textbf{0.449} & 0.802 / 0.445 &       -       &       -      \\
%	    \cline{1-7}
%	    \end{tabular*}
	    
\begin{tabular*}{\textwidth}{|p{3.5cm}|p{2.8cm}|p{1.5cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\cline{1-8}
Categories & Training dataset size & \# of classes & TextCNN & MoE & Ensemble & MoHE-1 & MoHE-2\\
\hhline{|=|==||=====|}
\multicolumn{8}{c}{\textbf{Sampling of categories from Rakuten Ichiba Product Catalog Dataset}} \\ \cline{1-8}
\multicolumn{3}{|c}{} & \multicolumn{5}{c|}{\textit{Head}} \\ \cline{1-8}
	    Home Decor & \makecell[r]{1260798} & \makecell[r]{310}                  & xx.yy/xx.yy & xx.yy/xx.yy & 0.871/0.776 & 0.868/0.773 & 0.870/0.778 \\ \cline{1-8}
	    Foods & \makecell[r]{461963} & \makecell[r]{880}                        & xx.yy/xx.yy & xx.yy/xx.yy & 0.785/0.742 & 0.784/0.739 & 0.784/0.742 \\ \cline{1-8}
	    Healthcare \& Med. Supplies & \makecell[r]{420776} & \makecell[r]{381}  & xx.yy/xx.yy & xx.yy/xx.yy & 0.843/0.770 & 0.841/0.767 & 0.842/0.770 \\ \cline{1-8}
\multicolumn{3}{|c}{} & \multicolumn{4}{c|}{\textit{Torso}} \\ \cline{1-8}
        Computers \& Networking & \makecell[r]{384861} & \makecell[r]{263}      & xx.yy/xx.yy & xx.yy/xx.yy & 0.861/0.688 & 0.859/0.688 & 0.860/0.685 \\ \cline{1-8}
	    Shoes & \makecell[r]{340078} & \makecell[r]{80}                         & xx.yy/xx.yy & xx.yy/xx.yy & 0.814/0.708 & 0.811/0.708 & 0.811/0.711 \\ \cline{1-8}
	    Beverages & \makecell[r]{178114} & \makecell[r]{42}                     & xx.yy/xx.yy & xx.yy/xx.yy & 0.896/0.802 & 0.894/0.799 & 0.896/0.800 \\ \cline{1-8}
\multicolumn{3}{|c}{} & \multicolumn{5}{c|}{\textit{Tail}} \\ \cline{1-8}
	    Professional Services & \makecell[r]{49964} & \makecell[r]{85}          & xx.yy/xx.yy & xx.yy/xx.yy & 0.942/0.799 & 0.939/0.793 & 0.942/0.799 \\ \cline{1-8}
	    Cars \& Motorcycles & \makecell[r]{7088} & \makecell[r]{217}            & xx.yy/xx.yy & xx.yy/xx.yy & 0.976/0.932 & 0.977/0.938 & 0.976/0.935 \\ \cline{1-8}
	    Fiber-Optic/Mobile Comm. & \makecell[r]{1937} & \makecell[r]{10}        & xx.yy/xx.yy & xx.yy/xx.yy & 0.956/0.790 & 0.957/0.821 & 0.962/0.859 \\ \cline{1-8}
\multicolumn{7}{c}{\textbf{Rakuten.com SIGIR'18 E-Com Workshop Data Challenge Dataset}} \\ \cline{1-8}
	    All categories & \makecell[r]{712761} & \makecell[r]{3008}              & xx.yy/xx.yy & xx.yy/xx.yy & 0.811/0.450 & 0.801/0.449 & 0.810/0.452 \\ \cline{1-8}
\end{tabular*}

==> src/tables/table-meta_performance_1level.tex <==
%	    \begin{tabular*}{\textwidth}{|c|c|c|c|c|c|c|c|}
%	    \cline{1-8}
%	     & Baseline & Shop ID & Tag ID & Shop/Tag ID & desc-append & desc-aux & Shop/Tag ID + desc-aux\\
%	    \hhline{|========|}
%	    \cline{1-8}
%	    Home Decor & 0.797 & 0.805 & 0.813 & 0.823 & 0.800 & 0.799 & 0.822 \\
%	    \cline{1-8}
%	    Foods & 0.756 & 0.758 & 0.765 & 0.774 & 0.756 & 0.757 & 0.778 \\
%	    \cline{1-8}
%	    Healthcare \& Med. Supplies & 0.772 & 0.807 & 0.799 & 0.822 & 0.814 & 0.816 & 0.830 \\
%	    \cline{1-8}
%	    Shoes & 0.731 & 0.734 & 0.735 & 0.749 & 0.742 & 0.743 & 0.749 \\
%	    \cline{1-8}
%	    Computers \& Networking & 0.721 & 0.726 & 0.704 & 0.724 & 0.714 & 0.706 & 0.724 \\
%	    \cline{1-8}
%	    Beverages & 0.837 & 0.834 & 0.844 & 0.852 & 0.836 & 0.839 & 0.861 \\
%	    \cline{1-8}
%	    Professional Services & 0.793 & 0.844 & 0.808 & 0.833 & 0.842 & 0.842 & 0.852 \\
%	    \cline{1-8}
%	    Cars \& Motorcycles & 0.923 & 0.900 & 0.918 & 0.905 & 0.903 & 0.903 & 0.923 \\
%	    \cline{1-8}
%	    Fiber-Optic/Mobile Comm. & 0.705 & 0.838 & 0.797 & 0.770 & 0.715 & 0.636 & 0.855 \\
%	    \cline{1-8}
%	    \end{tabular*}
	    
%	    \begin{tabular*}{\textwidth}{|c|c|c|c|c|c|c|}
%	    \cline{1-7}
%	     & Baseline & Shop ID & Tag ID & Shop/Tag ID & desc. & Shop/Tag ID + desc.\\
%	    \hhline{|=======|}
%	    \cline{1-7}
%	    Home Decor & 0.797 & 0.805 & 0.813 & 0.823 & 0.799 & 0.822 \\
%	    \cline{1-7}
%	    Foods & 0.756 & 0.758 & 0.765 & 0.774 & 0.757 & 0.778 \\
%	    \cline{1-7}
%	    Healthcare \& Med. Supplies & 0.772 & 0.807 & 0.799 & 0.822 & 0.816 & 0.830 \\
%	    \cline{1-7}
%	    Shoes & 0.731 & 0.734 & 0.735 & 0.749 & 0.743 & 0.749 \\
%	    \cline{1-7}
%	    Computers \& Networking & 0.721 & 0.726 & 0.704 & 0.724 & 0.706 & 0.724 \\
%	    \cline{1-7}
%	    Beverages & 0.837 & 0.834 & 0.844 & 0.852 & 0.839 & 0.861 \\
%	    \cline{1-7}
%	    Professional Services & 0.793 & 0.844 & 0.808 & 0.833 & 0.842 & 0.852 \\
%	    \cline{1-7}
%	    Cars \& Motorcycles & 0.923 & 0.900 & 0.918 & 0.905 & 0.903 & 0.923 \\
%	    \cline{1-7}
%	    Fiber-Optic/Mobile Comm. & 0.705 & 0.838 & 0.797 & 0.770 & 0.636 & 0.855 \\
%	   \hhline{|=======|}
%	    All 38 Genres, 2-level & 0.700 & 0.712 & 0.708 & 0.719 & 0.712 & 0.723 \\
%	    \cline{1-7}
%	    \end{tabular*}

%\begin{tabular*}{\textwidth}{|c|c|c|c|c|c|c|c|c|} \cline{1-9}
%& Data Size & N Class & Baseline & Shop ID & Tag ID & Shop/Tag ID & desc. & Shop/Tag ID + desc.\\
%\hhline{|=========|} \cline{1-9}
%Home Decor & \makecell[r]{1260798} & \makecell[r]{310} & 0.885 / 0.793 & 0.889 / 0.805 & 0.896 / 0.813 & 0.901 / \textbf{0.823} & 0.887 / 0.799 & \textbf{0.902} / 0.822 \\ \cline{1-9}
%Foods & \makecell[r]{461963} & \makecell[r]{880} & 0.794 / 0.746 & 0.805 / 0.758 & 0.808 / 0.765 & 0.819 / 0.774 & 0.802 / 0.757 & \textbf{0.820} / \textbf{0.778} \\ \cline{1-9}
%Healthcare \& Med. Supplies & \makecell[r]{420776} & \makecell[r]{381} & 0.854 / 0.788 & 0.871 / 0.807 & 0.861 / 0.799 & 0.879 / 0.822 & 0.873 / 0.816 & \textbf{0.886} / \textbf{0.830} \\ \cline{1-9}
%Shoes & \makecell[r]{340078} & \makecell[r]{80} & 0.827 / 0.728 & 0.833 / 0.734 & 0.839 / 0.735 & 0.844 / 0.749 & 0.834 / 0.743 & \textbf{0.845} / \textbf{0.753} \\ \cline{1-9}
%Computers \& Networking & \makecell[r]{384861} & \makecell[r]{263} & 0.875 / 0.698 & 0.886 / \textbf{0.726} & 0.879 / 0.704 & 0.890 / 0.724 & 0.882 / 0.706 & \textbf{0.891} / 0.724 \\ \cline{1-9}
%Beverages & \makecell[r]{178114} & \makecell[r]{42} & 0.902 / 0.832 & 0.909 / 0.834 & 0.922 / 0.844 & 0.925 / 0.852 & 0.910 / 0.839 & \textbf{0.928} / \textbf{0.861} \\ \cline{1-9}
%Professional Services & \makecell[r]{49964} & \makecell[r]{85} & 0.944 / 0.804 & 0.950 / 0.844 & 0.947 / 0.808 & 0.951 / 0.833 & 0.952 / 0.812 & \textbf{0.956} / \textbf{0.852} \\ \cline{1-9}
%Cars \& Motorcycles & \makecell[r]{7088} & \makecell[r]{217} & 0.960 / 0.897 & 0.969 / 0.900 & 0.965 / 0.918 & 0.969 / 0.905 & 0.965 / 0.903 & \textbf{0.975} / \textbf{0.923} \\ \cline{1-9}
%Fiber-Optic/Mobile Comm. & \makecell[r]{1937} & \makecell[r]{10} & 0.944 / 0.770 & 0.962 / 0.838 & 0.956 / 0.797 & 0.955 / 0.770 & 0.945 / 0.636 & \textbf{0.973} / \textbf{0.855} \\ \cline{1-9}
%\hhline{|=========|}
%All 38 Genres, 2-level & \makecell[r]{23701953} & \makecell[r]{11397} & 0.808 / 0.701 & 0.817 / 0.712 & 0.815 / 0.708 & 0.824 / 0.719 & 0.819 / 0.712 & \textbf{0.828} / \textbf{0.723} \\ \cline{1-9}
%\end{tabular*}

\begin{tabular*}{\textwidth}{p{3.5cm}|p{1.4cm}|p{0.9cm}||p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.4cm}} \cline{1-9}
Categories & Training data size & \# of classes & Baseline & Shop ID & Tag ID & Shop/Tag ID & desc. & Shop/Tag ID + desc.\\
\hhline{|=========|} \cline{1-9}
Home Decor & \makecell[r]{1260798} & \makecell[r]{310}                  & 0.886/0.798 & xx.yy & xx.yy & xx.yy & xx.yy & 0.898/0.811 \\ \cline{1-9}
Foods & \makecell[r]{461963} & \makecell[r]{880}                        & 0.799/0.752 & xx.yy & xx.yy & xx.yy & xx.yy & 0.814/0.760 \\ \cline{1-9}
Healthcare \& Med. Supplies & \makecell[r]{420776} & \makecell[r]{381}  & 0.857/0.788 & xx.yy & xx.yy & xx.yy & xx.yy & 0.882/0.823 \\ \cline{1-9}
\hhline{|=========|}
Shoes & \makecell[r]{340078} & \makecell[r]{80}                         & 0.829/0.733 & xx.yy & xx.yy & xx.yy & xx.yy & 0.843/0.747 \\ \cline{1-9}
Computers \& Networking & \makecell[r]{384861} & \makecell[r]{263}      & 0.877/0.701 & xx.yy & xx.yy & xx.yy & xx.yy & 0.888/0.720 \\ \cline{1-9}
Beverages & \makecell[r]{178114} & \makecell[r]{42}                     & 0.906/0.825 & xx.yy & xx.yy & xx.yy & xx.yy & 0.925/0.845 \\ \cline{1-9}
\hhline{|=========|}
Professional Services & \makecell[r]{49964} & \makecell[r]{85}          & 0.946/0.804 & xx.yy & xx.yy & xx.yy & xx.yy & 0.954/0.848 \\ \cline{1-9}
Cars \& Motorcycles & \makecell[r]{7088} & \makecell[r]{217}            & 0.971/0.912 & xx.yy & xx.yy & xx.yy & xx.yy & 0.976/0.903 \\ \cline{1-9}
Fiber-Optic/Mobile Comm. & \makecell[r]{1937} & \makecell[r]{10}        & 0.958/0.799 & xx.yy & xx.yy & xx.yy & xx.yy & 0.965/0.807 \\ \cline{1-9}
%\hhline{|=========|}
%All 38 Genres, 2-level & \makecell[r]{23701953} & \makecell[r]{11397}   & xx.yy & xx.yy & xx.yy & xx.yy & xx.yy & xx.yy \\ \cline{1-9}
\end{tabular*}

